Large-Scale Scenarios of Electric Vehicle Charging with a Data-Driven Model of Control

Planning to support widespread transportation electrification depends on detailed estimates for the electricity demand from electric vehicles in both uncontrolled and controlled or smart charging scenarios. We present a modeling approach to rapidly generate charging estimates that include control for large-scale scenarios with millions of individual drivers. We model uncontrolled charging demand using statistical representations of real charging sessions. We model the effect of load modulation control on aggregate charging profiles with a novel machine learning approach that replaces traditional optimization approaches. We demonstrate its performance modeling workplace charging control with multiple electricity rate schedules, achieving small errors (2.5% to 4.5%), while accelerating computations by more than 4000 times. We illustrate the methodology by generating scenarios for California's 2030 charging demand including multiple charging segments and controls, with scenarios run locally in under 50 seconds, and for assisting rate design modeling the large-scale impact of a new workplace charging rate.

==> arxiv_Large-Scale Scenarios of Electric Vehicle Charging with a Data-Driven Model of Control/table1.tex <==


% \include{table1}
\begin{table*}
\resizebox{\textwidth}{!}{%
 \begin{tabular}{||c| c c c c c c c c||} 
 \hline
 Rate & LR & Ridge & RF & MLP & Lin SVR & Quad SVR & RBF SVR & Sig SVR  \\ [0.5ex] 
 \hline\hline
 Peak Minimization & \cellcolor{shade1!70} 0.02558 & \cellcolor{shade1!70} \textbf{0.02508} & \cellcolor{shade1!70} 0.02612 & \cellcolor{shade2!70} 0.02724 & \cellcolor{shade1!70} \textbf{0.02492} & \cellcolor{shade1!70} 0.02518 & \cellcolor{shade1!70} 0.02505 & \cellcolor{shade2!70} 0.02835 \\
 \hline
 PG\&E CEV & \cellcolor{shade7!70} 0.04854 & \cellcolor{shade6!70} 0.04748 & \cellcolor{shade6!70} \textbf{0.04554} & \cellcolor{shade6!70} 0.04667 & \cellcolor{shade7!70} 0.04808 & \cellcolor{shade7!70} 0.05130 & \cellcolor{shade7!70} 0.05144 & \cellcolor{shade8!70} 0.05632 \\
 \hline
 PG\&E CEV demand only & \cellcolor{shade1!70} 0.02365 & \cellcolor{shade1!70} \textbf{0.02305} & \cellcolor{shade1!70} 0.02375 & \cellcolor{shade1!70} 0.02630 & \cellcolor{shade1!70} \textbf{0.02288} & \cellcolor{shade1!70} 0.02324 & \cellcolor{shade1!70} 0.02303 & \cellcolor{shade2!70} 0.02743 \\
\hline
 PG\&E CEV energy only & \cellcolor{shade6!70} 0.04598 & \cellcolor{shade6!70} 0.04461 & \cellcolor{shade5!70} \textbf{0.04352} & \cellcolor{shade6!70} 0.04743 & \cellcolor{shade6!70} 0.04476 & \cellcolor{shade6!70} 0.04640 & \cellcolor{shade6!70} 0.04626 & \cellcolor{shade7!70} 0.05207 \\
 \hline
 PG\&E E19 & \cellcolor{shade2!70} 0.02889 & \cellcolor{shade2!70} 0.02828 & \cellcolor{shade2!70} \textbf{0.02775}& \cellcolor{shade2!70} 0.03109& \cellcolor{shade2!70} 0.02865& \cellcolor{shade3!70} 0.03140 & \cellcolor{shade3!70} 0.03128& \cellcolor{shade3!70} 0.03537 \\
 \hline 
 SCE TOU-EV-8 & \cellcolor{shade3!70} 0.03399 & \cellcolor{shade3!70} \textbf{0.03290} & \cellcolor{shade4!70} 0.03958 & \cellcolor{shade4!70} 0.03768	& \cellcolor{shade3!70} 0.03330 & \cellcolor{shade3!70} 0.03499 & \cellcolor{shade3!70} 0.03509	& \cellcolor{shade6!70} 0.04414\\
 \hline
\end{tabular}} 
\caption{Root mean squared error (RMSE) on the test set reported for each functional form and rate schedule. The shading divides the range of values into 8 colors, with darker reds showing the worse results. Bold font is used to highlight the best result for each rate based on performance in either the test set or cross-validation.} 
\label{tab:error_results}
\end{table*}	

